Interactive Segmentation for COVID-19 Infection Quantification on Longitudinal CT scans

Consistent segmentation of COVID-19 patient's CT scans across multiple time points is essential to assess disease progression and response to therapy accurately. Existing automatic and interactive segmentation models for medical images only use data from a single time point (static). However, valuable segmentation information from previous time points is often not used to aid the segmentation of a patient's follow-up scans. Also, fully automatic segmentation techniques frequently produce results that would need further editing for clinical use. In this work, we propose a new single network model for interactive segmentation that fully utilizes all available past information to refine the segmentation of follow-up scans. In the first segmentation round, our model takes 3D volumes of medical images from two-time points (target and reference) as concatenated slices with the additional reference time point segmentation as a guide to segment the target scan. In subsequent segmentation refinement rounds, user feedback in the form of scribbles that correct the segmentation and the target's previous segmentation results are additionally fed into the model. This ensures that the segmentation information from previous refinement rounds is retained. Experimental results on our in-house multiclass longitudinal COVID-19 dataset show that the proposed model outperforms its static version and can assist in localizing COVID-19 infections in patient's follow-up scans.

==> glossary.tex <==
% Covid
\newacronym{ct}{CT}{computed tomography}
\newacronym{c19}{COVID-19}{coronavirus disease}
\newacronym{acons}{CONS}{consolidation}
\newacronym{aggo}{GGO}{ground glass opacity}
\newacronym{apleff}{PLEFF}{pleural effusion}

\newglossaryentry{ggo}
{
  name=ground glass opacity,
  description={\mbox{}\\* is the non-specific hazy opacification of the lung in \acrshort{ct} with no erasure of bronchial or vascular markings. The inferred pathology include partial filling of the lung alveoli by fluid, interstitial thickening, or partial collapse of lung alveoli \cite{Hodler2007}}
}

\newglossaryentry{cons}
{
  name=consolidation,
  description={\mbox{}\\* is defined as pathological alteration of lung tissue from an aerated condition to one of solid consistency through fluid, exudates, transudate, blood, or neoplastic cells \cite{Hansell2008} }
}
\newglossaryentry{pleff}
{
  name=pleural effusion,
  description={\mbox{}\\* is the build-up of excess fluid in the pleural space outside the lungs \cite{Zhan2021}}
}
